Star formation law in the EoR from [CII] and CIII] lines

We present a novel method to simultaneously characterise the star formation law and the interstellar medium properties of galaxies in the Epoch of Reionization (EoR) through the combination of [CII] 158$\mu$m (and its known relation with star formation rate) and CIII]$\lambda$1909{\AA} emission line data. The method, based on a Markov Chain Monte Carlo algorithm, allows to determine the target galaxy average density, $n$, gas metallicity, $Z$, and burstiness parameter, $\kappa_s$, quantifying deviations from the Kennicutt-Schmidt relation. As an application, we consider COS-3018 (z=6.854), the only EoR Lyman Break Galaxy so far detected in both [CII] and CIII]. We show that COS-3018 is a moderate starburst ($\kappa_s \approx 3$), with $Z\approx 0.4\, Z_{\odot}$, and $n \approx 500\, {\rm cm^{-3}}$. Our method will be optimally applied to joint ALMA and JWST targets.

==> pdflink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother


